Tri-Perspective View Decomposition for Geometry-Aware Depth Completion

Depth completion is a vital task for autonomous driving, as it involves reconstructing the precise 3D geometry of a scene from sparse and noisy depth measurements. However, most existing methods either rely only on 2D depth representations or directly incorporate raw 3D point clouds for compensation, which are still insufficient to capture the fine-grained 3D geometry of the scene. To address this challenge, we introduce Tri-Perspective view Decomposition (TPVD), a novel framework that can explicitly model 3D geometry. In particular, (1) TPVD ingeniously decomposes the original point cloud into three 2D views, one of which corresponds to the sparse depth input. (2) We design TPV Fusion to update the 2D TPV features through recurrent 2D-3D-2D aggregation, where a Distance-Aware Spherical Convolution (DASC) is applied. (3) By adaptively choosing TPV affinitive neighbors, the newly proposed Geometric Spatial Propagation Network (GSPN) further improves the geometric consistency. As a result, our TPVD outperforms existing methods on KITTI, NYUv2, and SUN RGBD. Furthermore, we build a novel depth completion dataset named TOFDC, which is acquired by the time-of-flight (TOF) sensor and the color camera on smartphones. Project page: https://yanzq95.github.io/projectpage/TOFDC/index.html

==> sec/X_suppl_non_ref.tex <==
\clearpage
\setcounter{page}{1}
\maketitlesupplementary


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{figure}[t]
  \centering
  \includegraphics[width=1\columnwidth]{point_distribution.pdf}\\
  \caption{Comparison of the common 3D cubic convolution and our proposed distance-aware spherical convolution. }\label{fig_pd}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\centering
% \footnotesize
\renewcommand\arraystretch{1.5}
\resizebox{0.478\textwidth}{!}{
\begin{tabular}{ll}
\toprule
\multicolumn{2}{l}{For one pixel $p$ in the valid pixel set $\mathbb{P}$: } \\ \midrule
-- REL               & $\frac{1}{|\mathbb{P}|}\sum\limits{{{\left| \mathbf y_{p}-{\mathbf x}_{p} \right|/{\mathbf y_{p}}}}}$  \\ 
-- MAE               & $\frac{1}{|\mathbb{P}|}\sum\limits{{{\left| \mathbf y_{p}-{\mathbf x}_{p} \right|}}}$  \\ 
-- iMAE              & $\frac{1}{|\mathbb{P}|}\sum\limits{{{\left| 1/{\mathbf y_{p}}-1/{{\mathbf x}_{p}} \right|}}}$  \\ 
-- RMSE              & $\sqrt{\frac{1}{|\mathbb{P}|}\sum\limits{{{\left( \mathbf y_{p}-{\mathbf x}_{p} \right)}}}^2}$  \\  
-- iRMSE             & $\sqrt{\frac{1}{|\mathbb{P}|}\sum\limits{{{\left( 1/{\mathbf y_{p}}-1/{{\mathbf x}_{p}} \right)}}}^2}$  \\  
-- RMSELog           & $\sqrt{\frac{1}{|\mathbb{P}|}\sum{{{\left(  {\log {\mathbf y}}-\log {\mathbf x} \right)}^{2}}}}$  \\  
-- ${\delta }_{i}$   & $\frac{|\mathbb{S}|}{|\mathbb{P}|}, \ \mathbb{S}: \max \left( {{\mathbf y_p}/{\mathbf x_p},{\mathbf x_p}/{\mathbf y_p}} \right)<{1.25}^{i}$  \\ 
\bottomrule
\end{tabular}
}
\caption{Definition of the seven metrics used in the main text.}\label{tab_metric}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\section{Distance-Aware Spherical Convolution}
\cref{fig_pd} illustrates the comparison of our distance-aware spherical convolution (DASC) and the 3D convolution. We observe that the $d$-relevant DASC involves a higher number of valid points with more balanced distribution. 



\section{Metric}
On KITTI benchmark, we employ RMSE, MAE, iRMSE, and iMAE for evaluation \cite{park2020nonlocal,zhou2023bev,wang2023lrru,yan2022rignet}. On NYUv2, TOFDC, and SUN RGBD datasets, RMSE, REL, and ${{\delta }_{i}}$ ($i=1, 2, 3$) are selected for testing \cite{Qiu_2019_CVPR,tang2020learning,zhang2023cf,yu2023aggregating}. 

For simplicity, let $\mathbf{x}$ and $\mathbf{y}$ denote the predicted depth and ground truth depth, respectively. \cref{tab_metric} defines the metrics. 


\section{Loss Function}
The total loss function $L_{total}$ consists of three terms, \textit{i.e.}, the front-view $L_f$, top-view $L_t$, and side-view $L_s$. The ground truths of the front, top, and side views are obtained by projecting the annotated point clouds. Following \cite{park2020nonlocal,lin2023dyspn,zhou2023bev}, we adopt $L_1$ and $L_2$ joint loss functions to denote $L_f$, $L_t$, and $L_s$, \textit{i.e.}, $L_f/L_t/L_s=L_1+L_2$. As a result, the total loss function $L_{total}$ is defined as: 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}\label{loss_function}
    L_{total}=L_f + \alpha L_t + \beta L_s,
\end{equation}
where $\alpha$ and $\beta$ are conducted to balance the three terms. Empirically, we set $\alpha$ and $\beta$ to 0.6 and 0.2, respectively. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\section{Implementation Detail}
We implement TPVD on Pytorch with four 3090 GPUs. We train it for 50 epochs with Adam \cite{Kingma2014Adam} optimizer. The initial learning rate is $5\times 10^{-4}$ for the first 30 epochs and is reduced to half for every 10 epochs. Following \cite{lin2023dyspn,wang2023lrru}, the stochastic depth strategy \cite{huang2016deep} is used for better training. Also, we employ color jitter and random horizontal flip for data augmentation. The batch size is 3 for each GPU. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[t]
\centering
\renewcommand\arraystretch{1.1}
\resizebox{0.87\textwidth}{!}{
\begin{tabular}{l|cc|c|c|ccc|c}
\toprule
Dataset     & Outdoor & Indoor  & Sensor  & Edge Device  & Train  & Test  & Resolution  & Real-world  \\ 
\midrule
KITTI \cite{Uhrig2017THREEDV}    & \checkmark & $\times$    & LiDAR       & $\times$  & 86,898  & 1,000  & $1216\ast 352$  & \checkmark  \\
NYUv2 \cite{silberman2012indoor} &  $\times$  & \checkmark  & Kinect TOF  & $\times$  & 47,584  & 654    & $304\ast 228$  & $\times$  \\
TOFDC                            & \checkmark & \checkmark  & Phone TOF   & \checkmark  & 10,000  & 560    & $512\ast 384$  & \checkmark  \\
\bottomrule
\end{tabular}
}
\vspace{-5pt}
\caption{Dataset comparison. Note that these characteristics are calculated according to the \textbf{depth completion task}.}\label{tab_dataset_comparison}
\vspace{-5pt}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{TOFDC}

\subsection{Motivation}
For depth completion task, the commonly used datasets are KITTI \cite{Uhrig2017THREEDV} and NYUv2 \cite{silberman2012indoor}. \cref{tab_dataset_comparison} lists the detailed characteristics. 
KITTI uses LiDAR to collect outdoor scenes, while NYUv2 employs Kinect with time-of-flight (TOF) to capture indoor scenes. However, both LiDAR and Kinect are bulky and inconvenient, especially for ordinary consumers in daily life. Recently, TOF depth sensors have become more common on edge devices (\textit{e.g.}, mobile phones), as depth information is vital for human-computer interaction, such as virtual reality and augmented reality. Therefore, it is important and worthwhile to create a new depth completion dataset on consumer-level edge devices.


\subsection{Data Collection}
\noindent \textbf{Acquisition System.} As illustrated in Fig. 5 (left), 
%\cref{collection_raw_data} (left), 
the acquisition system consists of the Huawei P30 Pro and Helios, which capture color image and raw depth, and ground truth depth, respectively. The color camera of P30 produces $3648\times 2736$ color images using a 40 megapixel Quad Bayer RYYB sensor, while the TOF camera outputs $240\times 180$ raw depth maps. The industrial-level Helios TOF camera generates higher-resolution depth. Their depth acquisition principle is the same, ensuring consistent depth values. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{figure}[t]
  \centering
  \includegraphics[width=1\columnwidth]{TOFDC_statistic_density_prob.pdf}\\
  \caption{Density-probability comparison of raw depth maps.}\label{tofdc_statistic_density_prob}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent \textbf{Data Processing.} We calibrate the RGB-D system of the P30 with the Helios TOF camera. We align them on the $640\times 480$ color image coordinate using the intrinsic and extrinsic parameters. The color images and Helios depth maps are cropped to $512\times 384$, while the P30 depth maps to $192\times 144$. Then we conduct nearest interpolation to upsample the P30 depth maps to $512\times 384$. For the Helios depth maps, there still exist some depth holes caused by environment and object materials (\textit{e.g.}, transparent glass). We use the colorization technique (Levin \textit{et. al}) to fill the holes. %\cref{collection_raw_data} (right) 
Fig. 5 (right) shows the visual result. 

\cref{tofdc_statistic_density_prob} provides the corresponding statistical support. It reveals that the depth density of NYUv2 varies mainly from 60\% to 80\%, whereas that of TOFDC is highly concentrated between 95\% and 100\%. 


As reported in \cref{tab_dataset_comparison}, we collect the new depth completion dataset TOFDC. It consists of indoor and outdoor scenes, including texture, flower, light, video, and open space in \cref{tofdc_examples}. For the depth completion task, we take the raw depth captured by the P30 TOF lens as input, which is different from NYUv2 where the input depth is sampled from the ground truths. 

\subsection{Cross-Dataset Evaluation}
To validate the generalization on indoor scenes~\cite{yu2023aggregating}, we train TPVD on NYUv2 and test it on SUN RGBD. Comparing Tab.~\ref{tab_sunrgbd}-Kinect with %Tab.~\ref{tab_nyuv2}, 
Tab. 3, the errors of all methods increase and the accuracy decreases due to different RGB-D sensors. When comparing Tab.~\ref{tab_sunrgbd}-Xtion with %Tab.~\ref{tab_nyuv2},
Tab. 3, since the data is from different Xtion devices, 
we discover that the performance drops by large margins. However, Tab.~\ref{tab_sunrgbd} reports that our TPVD still 
achieves the lowest errors and the highest accuracy under Kinect V1 and Xtion splits. For example, under Xtion split, the RMSE of TPVD is 9 mm superior to those of the second best NLSPN~\cite{park2020nonlocal} and PointDC~\cite{yu2023aggregating}. These facts evidence the powerful cross-dataset generalization ability of our TPVD. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\centering
\renewcommand\arraystretch{1.1}
\resizebox{0.478\textwidth}{!}{
\begin{tabular}{l|ccccc}
\toprule
Method          & RMSE (m) $\downarrow$      & REL $\downarrow$     &${\delta }_{1}$  $\uparrow$ & ${\delta }_{{2}}$ $\uparrow$ & ${\delta }_{{3}}$  $\uparrow$ \\ 
\midrule 
\multicolumn{6}{c}{Collected by Kinect V1} \\ 
\midrule 
CSPN \cite{2018Learning}          & 0.729    & 0.504   & 69.1  & 77.8  & 84.0  \\
NLSPN \cite{park2020nonlocal}     & 0.093    & 0.020   & 98.9  & 99.6  & 99.7  \\ 
CostDCNet \cite{kam2022costdcnet} & 0.119    & 0.033   & 98.1  & 99.6  & 99.7  \\ 
GraphCSPN \cite{liu2022graphcspn} & 0.094    & \textcolor{blue}{0.023}   & 98.8  & 99.6  & 99.7  \\ 
PointDC \cite{yu2023aggregating}  & \textcolor{blue}{0.092}    & \textcolor{blue}{0.023}   & 98.9  & 99.6  & 99.8  \\
%\midrule
\textbf{TPVD (ours) }             & \textbf{0.087}    & \textbf{0.022}   & \textbf{99.1}  & \textbf{99.7}  & \textbf{99.8}  \\
\midrule
\multicolumn{6}{c}{Collected by Xtion} \\ 
\midrule 
CSPN \cite{2018Learning}          & 0.490    & 0.179   & 84.5  & 91.5  & 95.1  \\
NLSPN \cite{park2020nonlocal}     & \textcolor{blue}{0.128}    & 0.015   & 99.0  & 99.7  & 99.9  \\ 
CostDCNet \cite{kam2022costdcnet} & 0.207    & 0.028   & 97.8  & 99.1  & 99.5  \\ 
GraphCSPN \cite{liu2022graphcspn} & 0.131    & 0.017   & 99.0  & 99.7  & 99.9  \\ 
PointDC \cite{yu2023aggregating}  & \textcolor{blue}{0.128}    & \textcolor{blue}{0.016}   & 99.1  & 99.7  & 99.9  \\
%\midrule
\textbf{TPVD (ours) }             & \textbf{0.119}    & \textbf{0.014}   & \textbf{99.3}  & \textbf{99.8}  & \textbf{99.9}  \\
\bottomrule
\end{tabular}
}
\vspace{-6pt}
\caption{Cross-dataset evaluation on SUN RGBD benchmark.}\label{tab_sunrgbd}
\vspace{-4pt}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{figure}[!ht]
  \centering
  \includegraphics[width=1\columnwidth]{TOFDC_examples.pdf}\\
  \vspace{-5pt}
  \caption{TOFDC examples in different scenarios.}\label{tofdc_examples}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
